Mobility Map Inference from Thermal Modeling of a Building

We consider the problem of inferring the mobility map, which is the distribution of the building occupants at each timestamp, from the temperatures of the rooms. We also want to explore the effects of noise in the temperature measurement, room layout, etc. in the reconstruction of the movement of people within the building. Our proposed algorithm tackles down the aforementioned challenges leveraging a parameter learner, the modified Least Square Estimator. In the absence of a complete data set with mobility map, room and ambient temperatures, and HVAC data in the public domain, we simulate a physics-based thermal model of the rooms in a building and evaluate the performance of our inference algorithm on this simulated data. We find an upper bound of the noise standard deviation (<= 1F) in the input temperature data of our model. Within this bound, our algorithm can reconstruct the mobility map with a reasonable reconstruction error. Our work can be used in a wide range of applications, for example, ensuring the physical security of office buildings, elderly and infant monitoring, building resources management, emergency building evacuation, and vulnerability assessment of HVAC data. Our work brings together multiple research areas, Thermal Modeling and Parameter Estimation, towards achieving a common goal of inferring the distribution of people within a large office building.

==> arxivMobility (2)/previous things/previous_equations.tex <==
\section{\label{sec:2}Simulation and Problem Formulation}
As we mentioned earlier, the goal of this paper is to infer Mob Map from the temperature data. Some very important factors needed for this purpose are building architecture, building occupants, temperature contribution by them, ambient temperature and HVAC states etc. Unfortunately, there is no single data set available which can incorporate all these factors together. So, for the lack of ground truth, we build a thermal model of the building taking all the above mentioned factors into account.

\textbf{Thermal model simulation: }Our model relies on the following principle:

Total heat flow in the room (in watts) = Heat flow resulting in `Change in Temperature' = Cooling/heating conduction due to external environmental temperature + Temperature variation due to heat conduction among neighbouring rooms + Heating from internal sources like computers , lights, printers etc. (in watts) + Heating from people in the room (in watts) + Temperature change due to air conditioning contribution.


So, the equation for cooling in the rooms will look like this:


Total heat flow in the room, $\dot{Q}_i^{total}= C_i \frac{dT_i}{dt}$
$$= a_{ext}(T_{ext}(t)-T_i (t)) +a_{rooms} \sum_{j \in neighbours}^{} (T_j(t)-T_i(t))$$ 
\begin{equation} \label{eq:1}
 + \dot{Q}_{internal} + \dot{Q}_i^{mob}(t) + \rho \dot{V}_{HVAC} C_p (T_{HVAC}(t)-T_i(t)) u_i(t)
\end{equation}
where,

$C_i$ is the Heat Capacity of room $i$.

$\frac{dT_i}{dt}$ is the rate of temperature change in room $i$.

$T_i (t)$ is the Temperature of room $i$ at time $t$.

$a_{ext}$ and $a_{rooms}$ are constants related to heat conduction.

$T^{external} (t)$ is the ambient temperature at time $t$.

$\dot{Q}_{internal}$ is the heating due to internal devices. We have considered this constant across all rooms in a building.

$\dot{Q}_i^{mob}(t)$ is the heating due to mob present in the room $i$ at time $t$.

$\rho$ is the air conditioning air density.

$\dot{V}_{HVAC}$ is (volume/time) of cool air coming in. We have considered this constant across all rooms.

$C_p$ is the specific heat capacity of cool air.

$T_{HVAC}$ is the temperature of cool air. For bigger rooms, we have considered cool air having lower temperature.

$u_i(t)$ is the air-condition controller input( mainly ON/OFF).

Now we go into the details of each term and assumptions made for each term one by one.

\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=5cm]{tex.png}
    \caption{July,2019 daily ambient external temperature data in Marceed, CA. Average daily temperature in Marceed, CA in red dots. }
    \label{fig:tex}
\end{figure}
\textbf{(i) Generation of $T_{ext}(t)$}: Generation of External ambient temperature is a bit tricky because temperature varies a lot depending on the season, daily time and place. For this simulation, we have focused on cooling mainly. Therefore, we are simulating an environment where the ambient temperature is relatively higher so that the cooling system can trigger. We could have generated a Multivariate Normal Distribution with non-trivial co-variance matrix to generate the ambient temperature. But to include a practical real world experience, we have considered the ambient temperature data of Marceed, California during summer time. We have taken the average temperature at each moment(actually at time step, $\Delta t= 5$ minutes interval) for 10 hours daily over 1 month data. Fig. \ref{fig:tex} will demonstrate the whole July,2019 data from 9:00 to 19:00 and also show the average ambient temperature at each time step. The mean and standard deviation of the average data are 85F and 4.33 respectively. The data can be found from \cite{bell2013us}.

\textbf{(ii) Generation of $\dot{Q}_{internal}$}: This term is responsible for heat generation inside the rooms. Typically, we can see 3 computers, 1 printer, 4 light bulbs in a room. The temperature contribution by these devices is presented in Section \ref{subsec:supli1}. Other heating sources, such as Heaters, may also be present inside the rooms. But as we have stated earlier, since we are simulating a `Cooling down' environment, we are ignoring the Heater in this simulation. Nonetheless, our map Reconstruction Algorithm, discussed in Section \ref{sec:3}, can detect other possible heating sources if present.

\textbf{(iii) Generation of $\dot{Q}_i^{mob}(t)$}: This term refers to the heat generation from the occupants' body. We have considered that the number of people in a room is \textit{constant} for an hour. That means, after people come inside an office room, they do not go out at least for an hour. This time (here 1 hour) is called \textit{Time Range\textbf{(TR)}} between which mob number stays \textit{constant} at every room. More about TR is discussed in \ref{sec:4}. Also, for now, we are assuming that total number of people, $N$, in all $k$ rooms of the building is fixed over any time. That means, if the number of people in room $i$ at time $t$ is $n_i(t)$ then:
\[
    \sum_{i=1}^{k} n_i (t) = N\\
\]

Now, the heat contribution by the mobs in room $i$ , 
$$\dot{Q}_i^{mob}(t) = \sum_{m=1}^{m=n_i(t)} <q_m>$$
where, $<q>$ is the emitted energy distribution from mobs' body [$<q>=Gaussian(\mu = 110W, \sigma=1$)]

\textbf{(iv) Generation of $n_i(t)$}: Let, number of big conference room = BCR; number of small conference room = SCR and number of office rooms = OR. In our simulation model, we have assumed that BCR=1; SCR=1 and OR=14.

Let, the number of people staying in room $i$ will depend on some weight, $w_i$. [ to simulate the situation that conference rooms generally contain more people than the office rooms] 

So, the probability that a person will stay in room $i$ = $\frac{w_i}{\sum_{i} w_i}$ where, weight vector, $W = [w_1,w_2,......., w_N] = w_{1}^{b},w_{BCR+1}^{s}, w_{BCR+SCR+1}^{o}....,w_{N-BCR+SCR}^{o}.  $
Here, $w_{i}^{b}$ is the weight for big conference room, $w_{i}^{s}$ is the weight for small conference room and $w_{i}^{o}$ is the weight for office rooms. Choice of $W$ is mentioned in \ref{subsec:supli2}.\newline

\textbf{(v) Generation of $T_{HVAC}$}: We have assumed that the HVAC supplies cool air with temperature \textit{constant} over the times but variable across rooms. For instance, in our simulation, we have considered $T_{HVAC}$ = 50F for  big conference room and 55F for small conference or office rooms.

\textbf{(vi) Generation of $u_i(t)$}: This term refers to the ON/OFF state of HVAC's AC system. Depending on the current temperature of a room, the HVAC can trigger the AC system. Usually the occupants prefer their room temperature in a comfortable range. Therefore, the set points of room temperatures $T_i \in [T_i^{min}, T_i^{max}]$ and depending on that the AC controller input:
\[
    u_i(t)= 
\begin{cases}
    1,& \text{if } T_i\geq T_i^{max}\\
    0,& \text{if } T_i\leq T_i^{min}\\
    u_i(t-1),              & \text{otherwise}
\end{cases}
\]

where, $[T_i^{min} , T_i^{max}]$ is the temperature range in the rooms. 

\textbf{Final Simulation: }So far we have described the details about various factors present in Eq. (\ref{eq:1}). More details and calculations of these factors are given in \ref{subsec:supli1} and \ref{subsec:supli2}. Now, if we rewrite Eq. (\ref{eq:1}), the final equation that we are going to use looks like this:
$$\frac{T_i(t+1)-T_i(t)}{\Delta t} = \alpha (T_{ext}(t)-T_i (t)) + \beta \sum_{j \in X}^{} (T_j(t)-T_i(t)) +$$
\begin{equation} \label{eq:2}
 +  \omega + \gamma * M_{i}^{mob}(t) + \phi (T_{HVAC}(t)-T_i(t)) u_i(t)
\end{equation}
where,

$X$ is the set of neighbour rooms of room $i$.

$\alpha = \frac{a_{ext}}{C_i}$,$\beta = \frac{a_{rooms}}{C_i}$,$\omega = \frac{\dot{Q}_{internal}}{C_i} $,$\gamma = \frac{1}{C_i}$

$M_{i}^{mob}(t)=\sum_{m=1}^{m=n_i(t)} <q_m>$

$\phi = \frac{\rho \dot{V}_{HVAC} C_p}{C_i}$\newline

$\frac{dT_i}{dt}=\frac{T_i(t+1)-T_i(t)}{\Delta t}$ where $\Delta t$ is the time step which is the interval at which the sensor data is collected.

One thing to mention that we have performed 10 hours of
simulation. The time unit in our simulation will be in hour(h). Also we have run our simulator with all the temperature values in Kelvin($K$). For better understanding, we are mentioning the temperatures in Fahrenheit(F) in this paper. Finally, running our simulation, considering the parameters mentioned above and in \ref{subsec:supli1} and \ref{subsec:supli1}, the resulting outcomes following Eq. (\ref{eq:2}) can be viewed from Fig. \ref{fig:room1sensortempheattransfer}. The building architecture for our work is presented in Fig \ref{fig:architecture} as well.
\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=5cm]{architecture1.png}
    \caption{Architecture of the building for our simulation where we have a total of 16 rooms (Room 1- Big Conference room, Room 16- Small Conference room, Room 2 to 15- Normal Office room). We have assumed that Room 6,7,10 and 11 can exchange heat with only neighbouring rooms where as other rooms can exchange heat between both ambient and neighbouring rooms.}
    \label{fig:architecture}
\end{figure}

\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=5cm]{simulation1.png}
    \caption{Big conference room (Room 1) and  Office Room's (Room 2) Sensor Temperature Reading from our simulation (above) and other simulation factors such as mob distribution (mid) and AC controller input(below - 1 means ON).}
    \label{fig:room1sensortempheattransfer}
\end{figure}

From Fig. \ref{fig:room1sensortempheattransfer}, we can see that the temperatures are remaining between the set points (70F and 80F). Similar kind of behavior was observed in Ref. \cite{privara2013building} and \cite{hazyuk2012optimal} with a slight variation as we have taken building occupants and some other extra factors into account. Therefore, we can be confident that the temperature data from our simulation is completely valid.

\textbf{Problem formulation: }Now that we have simulation data of room temperatures in our hand, our problem formulation will be very easy. If we are given the temperature data of rooms and environment from temperature sensors, containing Gaussian noise, and AC's states from AHU sensors, using some known constants, \textbf{``Can we infer $M_{i}^{mob}(t)$ which is equivalent to infer $n_{i}^{mob}(t)$ correctly''?}  









%%%%%%%%%%%%%%%%% METHOD DESCRIPTION %%%%%%%%%%%%%%%%%%%%%


\section{\label{sec:3}Our Method to Infer Mob Map}
At this point we have our problem formulation. In this section, we will describe our map \textbf{Reconstruction Algorithm (RA)}. As stated earlier, our Algorithm is based on a variation of Least Square Estimator(LSE) with $L_2$ Regularization. LSE gives us our desired $M_{i}^{mob}(t)$ from which we can infer $n_{i}^{mob}(t)$ and $L_2$ regularization ensures the fact that the mobs stay at the same room for quite a moment. Now we will explain the development of our Algorithm step by step from the next paragraph.

\textbf{Development of our method: }If we rewrite Eq. (\ref{eq:2}) in matrix format for $k$ rooms and dividing it to L.H.S. and R.H.S we get:

L = $\frac{\Bar{T}(t+1)-\Bar{T}(t)}{\Delta t}$

R = $\alpha I  (\Bar{T}^{external} (t)-\Bar{T} (t)) + \beta I \sum ( \Bar{T}^{neighbour} (t) -\Bar{T} (t)) + \omega +  \gamma I \Bar{M}^{mob} (t) - \phi I (\Bar{T}_{HVAC}(t)- \Bar{T}(t)) \Bar{u}(t)$

The known things in our method are $C_i , \gamma, \phi$ and all other things are unknown. Among the unknowns, we are assuming that we can measure $ u_i$ (HVAC ON/OFF) without any noise. But this is not the case for $T_{HVAC}, T_i , T_{j \in Neighbour}$ and $T_{ext}$. So, assuming that we have some independent sensors which can measure these values with some Gaussian noises like:
\[
    \Bar{T}_{sensor} = \Bar{T} + Noise(\Bar{\eta})%\text{ and }
    %\Bar{T}_{sensor}^{external} = \Bar{T}_{ext} + \Bar{\eta}\\
\]
and put them in Eq. (\ref{eq:2}), we will get $L = R+ \eta$.
Therefore, if we want to find the Mob Map, we need to estimate the model parameters. For this, we will be using Least Square Estimation to decouple the noise ($\eta$) and optimize the model parameters $\alpha, \beta, \omega$ and $ \gamma \Bar{M}^{mob} (t)$. The procedure will look like this:
\begin{equation}\label{eq:3}
\begin{aligned}
& \underset{\alpha, \beta, \omega, \gamma \Bar{M}^{mob} (t) }{\text{argmin}}
& & \left\lVert L-R \right\rVert_{2}^{2} \\
& \text{s.t.} & &  \sum_{i=1}^{K} \gamma M_i^{mob}(t) = N*<\dot{q}>* \gamma \\
& & & \gamma* M_i^{mob}(t)\geq 0, \;  \forall i,t \\
\end{aligned}
\end{equation}

where $<\dot{q}>$ is the average energy emitted from a mob body. Now if we add $L_2$ Regularization term with (\ref{eq:3}) we can impose the situation where the number of mob remains almost same between two consecutive time steps.

\begin{equation}\label{eq:4}
\begin{aligned}
& \underset{P}{\text{argmin}}
& & \left\lVert L-R \right\rVert_{2}^{2}+\sum_{i=1}^{K}\sum_{t} \lambda \Bigg(M_i^{mob}(t+1)- M_i^{mob}(t)\Bigg)^2 \\
& & &   \\
\end{aligned}
\end{equation}
s.t. above constraints in (\ref{eq:3}). Here, $P=$ {$\alpha$, $\beta$, $ \omega$, $\gamma \Bar{M}^{mob} (t)$} and $\lambda = 0.1$.

The choice of $\lambda$ will be discussed in Section \ref{sec:4}. One thing to mention that if we have $k$ rooms and $z$ number of time steps (meaning that for each room we have collected the sensor data for z times at $\Delta t$ time interval, there are $P=k*z$ equations in this system. But we have $Q=k*z+3$ parameters to optimize. That means as P gets bigger, we get $P \approx Q$ which suggests that LSE will yield better convex solutions. 

\textbf{Relaxing the constraint: } We now focus on relaxing the constraint. The constraint in Eq. (\ref{eq:3}) mainly imposes that we need to know the exact total number of people inside the building to get the Mob Map which is hard to know. At most we can have a good guess on the total number of people in the building. We, now, rewrite this constraint in Eq. (\ref{eq:3})  which gives us the Mob Map if we can have a close guess on the total number of mob.
\begin{equation}\label{eq:5}
\begin{split}
N_{min}*\gamma<\dot{q}> \leq\sum_{i=1}^{K} \gamma M_i^{mob}(t)\leq N_{max}*\gamma <\dot{q}> =>\\
(1-\epsilon_2)N*\gamma<\dot{q}> \leq\sum_{i=1}^{K} \gamma M_i^{mob}(t)\leq (1+\epsilon_1)N*\gamma <\dot{q}>
\end{split}
\end{equation}
where, $\epsilon_1,\epsilon_2\geq0$. So, even if we specify a range of total mob, $[N_{min},N_{max}]$, in this constraint, we still get a reliable Mob Map. Note that if $\epsilon_2>1$, we have ignored the $(1-\epsilon_2)N*\gamma<\dot{q}>$ part because energy can not be negative. The effect of choosing $\epsilon_1$ and $\epsilon_2$ will be demonstrated in Section \ref{sec:4}.

However, we have now all the ingredients in our hand to run the estimator and it gives us the optimized parameter $\gamma \Bar{M}^{mob} (t)$ . The final rule used by our Reconstruction Algorithm to get $n_{i}^{mob}(t)$ is given below:
\begin{equation}\label{eq:6}
\text{Mob Map, }n_{i}^{mob}(t)=\text{Round to Integer}\left(\frac{\gamma* \Bar{M}^{mob} (t)}{\gamma * <\dot{q}>}\right)
\end{equation}

It can easily be seen that the performance of our Reconstruction Algorithm depends on $\epsilon, \lambda \text{ and } \eta$ whose effect will be discussed in Section \ref{sec:4}.









%%%%%%%%%%%%%%%%%%%%% RESULTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\label{sec:4}Results}
Now that we have described our Simulation, Problem Formulation and our Reconstruction Algorithm (\textbf{RA}), in this section, we show-case the output and performance of RA as well as the effect of various model parameters ($\epsilon, \lambda \text{ and } \eta$). 

\textbf{Output of RA applied on simulated temperature data: }
If we apply RA on the simulated data using Eq. (\ref{eq:4}) and (\ref{eq:6}), we can successfully recover the  model parameters, $\alpha, \beta, \omega, \gamma M_i^{mob}(t)$ and finally get $n_i^{mob}(t)$. We have recovered:

$$\alpha = 0.099  \text{ , } \beta = 0.101 \text{ and } \omega = 1.35$$ which is almost exact to the parameters used in simulation.

\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=6cm]{noisevsinference.png}
    \caption{Big conference room's (Room 1) Mob Map from simulated model and inferred parameter from RA at each hour for (a) Noise std, $\eta_{std}=10$  (b) $\eta_{std}=1$ (c) $\eta_{std}=0.1$ (d) $\eta_{std}=0.01$ [K=16, N= 45, BCR=1, SCR=1, OR=14 , $\Delta t=1 minute$, $z=600$, $TR=1$ hour, $\lambda=0.1$, $\epsilon=0.2$]}
    \label{fig:mobmapsunburstheattransfer}
\end{figure}


Fig. \ref{fig:mobmapsunburstheattransfer} demonstrates our constructed Mob Map, $n_i^{mob}(t)$, using Eq. (\ref{eq:6}) with the variation of noise. Note that, originally, for a room, we get the number of people at each time step. But usually people do not move from one room to another very often. For this, we defined \textit{Time Range(\textbf{TR})}, consisted of multiple time steps, in between no mob moves from one room to another. In our simulation, we assumed that mobs stay in one room for one hour, setting TR=1hour. So, in the final Mob Map construction, we took the Median of mob number over one hour. That is how we got one single mob number for each hour in Fig. \ref{fig:mobmapsunburstheattransfer}. When we implemented RA on real data set, we set TR=30 minutes and yet got reasonable mob map (shown later of this Section). In RA, TR can be set to any value depending on the situations and applications. However, we can see from Fig. \ref{fig:mobmapsunburstheattransfer} that when the standard deviation of noise is very high ($\eta_{std}=10$) in (a), the optimizer works very bad to infer the mob number. But as long as we decrease $\eta_{std}$ in (b), (c) and (d), the inference tends to match with the number of mob from our simulation. And finally at (d), when the $\eta_{std}=0.01$, the inferred mob number and simulated mob number are close to be matched.    

\textbf{Performace evaluation of RA: }
We measure the inference performance of RA by a term called \textit{Total Reconstruction Error \textbf{(TRE)}} which is a function of \textit{Normalized Mean Absolute Error \textbf{(NMAE)}}. The lower the TRE is, the better the performance is. We define TRE and NMAE as follows:

\[
    \text{TRE} = \frac{\sum_{i}^{k} \text{NMAE}_i}{k}\\
\]
\[
    \text{NMAE}_i = \frac{\text{Mean}(|Mob_{simulated} - Mob_{inferred}|_{\forall t})}{\text{Mean }Mob_{simulated} \text{ in room }i}\\
\]
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=4cm]{noisevserror.png}
    \caption{TRE of RA vs $Log_{10}$ of $\eta_{std}$ [K=16, N= 45, $\Delta t=1$ minute, $z=600$, $\lambda=0.1$, $\epsilon=0.2$].  }
    \label{fig:mobmapNMAEheattransfer}
\end{figure}
We measure the performance of RA on the basis of TRE with respect to the variation of the model parameters (i)$\eta_{std}$ ,(ii)$\lambda$ and (iii) $\epsilon$.

\textbf{(i) Effect of $\eta_{std}$ on TRE: }
Fig. \ref{fig:mobmapNMAEheattransfer} exhibits the effect of  $\eta_{std}$ (actually $Log_{10}$ of $\eta_{std}$)  on the performance of RA in terms of TRE. When $\eta_{std}\leq 1$ ($\leq $0 along X axis), we get TRE $\leq 0.2$ which is similar to having maximum 20\% error in reconstruction. If we consider that as our tolerance level, we can allow maximum Gaussian noise with standard deviation 1. Beyond that standard deviation, the reconstruction performance will degrade largely. Therefore, we recommend the level of accepted $\eta_{std}$ in range [0,1] to have a reliable Mob Map. 

\textbf{(ii) Effect of $\epsilon$ on TRE: }In Section \ref{sec:3}, we mentioned that our inference performance varies depending on the choice of $\epsilon_1$ and $\epsilon_2$ in constraint (\ref{eq:5}). We will show the effect of choosing $\epsilon_1$ and $\epsilon_2$ by considering $\epsilon_1=\epsilon_2=\epsilon$ which is equivalent to setting constraint $(1-\epsilon)N*\gamma<\dot{q}> \leq\sum_{i=1}^{K} \gamma M_i^{mob}(t)\leq (1+\epsilon)N*\gamma <\dot{q}>$. In Fig. \ref{fig:epsilonvstre}, we have shown the effect of $\epsilon$ on TRE. It is evident from Fig. \ref{fig:epsilonvstre} that choosing small range of $[N_{min},N_{max}](\epsilon \approx 0)$, closer to the actual total mob in the building yield better map reconstruction (lower TRE).  $\epsilon=0$ is equivalent to using the constraint in (\ref{eq:3}) as if we know the exact number of people in the building and in this case, the TRE is the lowest. Having $\epsilon>2$ is actually equivalent to using no constraint at all. So, the lower the $\epsilon$ be, the better the performance of RA be.  
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=4cm]{epsilonvstre.png}
    \caption{TRE of RA vs $\epsilon$ [K=16, N= 45, $\Delta t=1 minute$, $z=600$, $\lambda=0.1$, $\eta_{std}=0.1$].}
    \label{fig:epsilonvstre}
\end{figure}

\textbf{(iii) Effect of $\lambda$ on TRE: }The last thing we want to discuss is the effect of $\lambda$ on map reconstruction performance. From the empirical result shown in Fig. \ref{fig:lambdavstre}, we see that when $\lambda=0.1$, we get the lowest TRE, meaning better reconstruction. We recommend to use  $\lambda=0.1$ but depending on the recommended max tolerance level (20\%), $\lambda$ can have a value in range $\lambda=[0.03,0.3]$
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=4cm]{lambdavserror.png}
    \caption{TRE of RA vs $\lambda$ [K=16, N= 45, $\Delta t=1$ minute, $z=600$, $\epsilon=0.2$, $\eta_{std}=0.1$].}
    \label{fig:lambdavstre}
\end{figure}

\textbf{Implementation on Real Data set:}
As we have mentioned earlier, no data set is complete to run our method. That is why we choose to simulate the room temperatures. Till now we have seen the performance of RA on the simulated data. However, to show the effectiveness of RA in different scenario, we are implementing our method of RA to some real toy data sets. We assume reasonable values for the missing arguments for our Algorithm.

\textbf{(i) Data set 1:} This data, in \cite{armknecht2019privacy}, was collected from March to April, 2016. We have filtered the data set to get 10 hours of data(sampled every 3 minutes) from April 28, 2016 . It contains the temperature of only one room as well as the number of occupants in that room. As a consequence, we get ground truth to compare our results. The only problem of this data set is that we do not have some other distributions like ambient temperatures and HVAC status (ON/OFF or cool air temperature). We assume reasonable values for these. For example, we set $T_{ext}(t)$ from a distribution $(\mu=55F, \sigma=2)$ which is compatible with ambient temperature in Mannheim, Germany from where the data was collected. Another thing is that because of the average ambient temperature being very cool($\mu=55F$), we assume that the air conditioner is OFF. Considering these situations in mind, we have applied RA on this data set and got the Mob Map like in Fig. \ref{fig:germany}. Moreover, the relative higher value of $\omega = 2.31$ (in our simulation $\omega \text{was} 1.36$) delivered by RA indicates the presence of possible Heating System inside the room. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=4cm]{mobmap_germany.png} 
    \caption{Mob Map generated from Data set 1 ($TR=30$ minutes). At each TR, left column is our inferred mob number and right column is the actual mob number.[$\Delta t=3$ minutes, $z=200$, $\epsilon=0.2$, $\lambda=0.1$]}
    \label{fig:germany}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=4cm]{mobmap_house.png} 
    \caption{Mob Map generated from Data set 2 ($TR=30$ minutes).[$\Delta t=3$ minutes, $z=200$, $\epsilon=0.2$, $\lambda=0.1$]}
    \label{fig:house}
\end{figure}

\textbf{(ii) Data set 2:} We have filtered this data set in \cite{candanedo2017data} to collect 10 hours (9:00 to 19:00) of data sampled in every 10 minutes from May 26, 2016. The room architecture (neighbour room information) is known and we have gathered the data of all four rooms in lower floor. However, we can get $T_{ext}(t)$ and $T_i(t)$ directly from the data set. To get an idea of AC's ON/OFF status, we have observed that, for Room 3, the temperature dropped abruptly from 11:00 to 12:30 and from 14:00 to 17:00. We have assumed that in this time the AC was ON. Another thing is that there was no hints given about HVAC's air volume capacity or temperature of the cooled air. For this, we have used the values of $\phi$ and $T_{HVAC}$ from our simulation. Considering these assumptions, we have run RA on this data set and got the Mob Map of Room 3 similar to Fig. \ref{fig:house}. Note that there is no ground truth on the number of occupant in this data set. We have chosen Room 3 to show the Mob Map here because this room is attached with Room 1 and Room 2 as well as with the environment which is almost similar to our simulation design.  


%%%%%%%%%%%%%%%%%%%%%%%% DISCUSSION AND CONCLUSION %%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\label{sec:5}Discussion and Conclusion}
In this paper, we have simulated a thermal modeling of a building and proposed a method to infer the Mob Map. We have found out that if we have access to a particular room temperature, temperature of its neighbourhood rooms as well as AC's control dynamics such as ON/OFF status and cooled air temperature, we can easily infer a reliable Mob Map. Not only that, we also demonstrate the applicability and performance of RA in terms of Total Reconstruction Error with respect to the variation of various factors such as noise level from sensor data, choice of the constraint and other model parameters ($\epsilon , \lambda$) etc. Moreover, we have illustrated the effectiveness of our Algorithm by applying it on two test data sets. Still there are possible spaces for further development. In future, we will apply our method on a real data set compatible with our method. Another thing to mention that though our simulation model is moderately complex, there is still room for constructing more complex and realistic thermal model, for instance , accumulating solar radiation and heat transfer via convection.  





%%%%%%%%%%%%%%%%% SUPLIMENTARY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{\label{sec:6}Supplementary Materials}
\subsection{Choice of the Constants:}\label{subsec:supli1}
\textbf{$C_i$}: $C_i$ is the Heat Capacity for entire room. All the elements (air, furniture and walls) in a room contribute to it.
$$C_i= C_{air} + C_{furniture} + C_{wall} = (C_{volumetric}* volume) +$$ 
$$+(\text{Furniture mass * Specific Heat Capacity,}C_p ) + $$
$$+(\rho_{wall}*volume_{wall}*(C_p)_{wall})$$
Considering standard values, we get,
$$C_i=(1.29KJm^{-3}K^{-1} * 30m^3) + (4200 J/kgK * 200kg) +$$ $$+(2.13*10^5 gm^{-3}*5m^3*0.84 J/gK) = 1*10^6 J/K$$
$a_{ext}$: Every room performs heat transfer with the ambient temperature via conduction process in the wall and window glass. The equation for $a_{ext}$ is:
$$a_{ext} = h_{wall}*A_{wall} + h_{glass}*A_{glass}$$
where, h is the Thermal Transmittance of a substance. Using standard values we get:
$$a_{ext} = (1Wm^{-2}K^{-1} * 20m^2)+(5Wm^{-2}K^{-1} * 2m^2) = 30W/K$$

$a_{room}$: Every room performs heat transfer with neighbouring rooms via conduction process in the wall only. The equation is same as $a_{ext}$ but excluding the glass part. Using standard values we get:
$$a_{rooms} = (1Wm^{-2}K^{-1} * 20m^2) = 20W/K$$\newline


$\dot{Q}_{internal}$: Considering 3 computers (100W energy consumed per computer), 4 lights (10 W per light) and 1 printer(40W/printer) per room, each room will radiate a total of 380W = $1.36*10^6$J/h energy.\newline

$<\dot{q}>$: Average heat produced by an average human body while staying indoor is given by the equation:
$$<\dot{q}> = M*A_{body}$$
Considering standard Metabolic rate, $M = 55Wm^{-2}$ and average body area, $A_{body} = 2 m^2$ we get, $<\dot{q}> = 110W = 3.96*10^5 J/h$\newline

$\rho \dot{V}_{HVAC} C_p$: Considering each room 250 sqr-ft and standard rules of 1 Cubic ft per minute (1 CFM) per sqr-ft, we get $\dot{V}_{HVAC} = 250 CFM = 450 m^3/h$. Using usual values, we get $\rho \dot{V}_{HVAC} C_p$ = $\rho_{air} \dot{V}_{HVAC} (C_p)_{air}= 1.225 kgm^{-3} * 450 m^3/h *  1000 J/kgK = 5.51*10^5 J/hK$


Now,
$\alpha = \frac{a_{ext}}{C_i} = \frac{30W/K}{10^6 J/K}= 0.1h^{-1}$

$\beta = \frac{a_{rooms}}{C_i} = \frac{20W/K}{10^6 J/K}= 0.1h^{-1}$

$\omega = \frac{\dot{Q}_{internal}}{C_i} = \frac{1.36*10^6J/h}{10^6 J/K}=1.36 Kh^{-1}$

$\gamma = \frac{1}{C_i} = \frac{1}{10^6 J/K}= 10^{-6} K/J$

$\phi = \frac{\rho \dot{V}_{HVAC} C_p}{C_i} = \frac{5.51*10^5 J/hK}{10^6 J/K}= 0.6h^{-1}$\newline

\subsection{Simulation Parameters:}\label{subsec:supli2}

$\alpha = 0.1h^{-1}$, $\beta = 0.1h^{-1}$, $\omega =1.36 Kh^{-1}$, $\gamma = 10^{-6}KJ^{-1}$, $\phi = 0.6h^{-1}$

$[T_i^{min},T_i^{max}] = [70F, 80F]$

Total number of rooms, $k$ = 16 and Total mob in the building, $N$ = 45 [Distributed over $k$ rooms]

Number of Big Conference room, BCR = 1; number of Small Conference room, SCR = 1; number of Normal Office room, OR = 14.

Weight for Big conference room, $w_{i}^{b}$ = 5; weight for small conference room, $w_{i}^{s}$ = 3; weight for office room, $w_{i}^{o}$ = 1

Total time for simulation = 10 hours; time step for solving the equation, $\Delta t$ = 10/600 hour = 1 minute; Time range, $TR=1$ hour.

\subsection{Implementation Platform Details:}\label{subsec:supli3}
We have used Python platform (Python 3.7.2) and SQSLP optimization algorithm from  scipy package in order to manipulate the LSE and $L_2$ Regularization to  optimize the model parameters. All the codes were run in Macbook Pro, 2017, 2.3 GHz Intel Core i5, 16 GB memory. 


==> previous things/previous_equations.tex <==
\section{\label{sec:2}Simulation and Problem Formulation}
As we mentioned earlier, the goal of this paper is to infer Mob Map from the temperature data. Some very important factors needed for this purpose are building architecture, building occupants, temperature contribution by them, ambient temperature and HVAC states etc. Unfortunately, there is no single data set available which can incorporate all these factors together. So, for the lack of ground truth, we build a thermal model of the building taking all the above mentioned factors into account.

\textbf{Thermal model simulation: }Our model relies on the following principle:

Total heat flow in the room (in watts) = Heat flow resulting in `Change in Temperature' = Cooling/heating conduction due to external environmental temperature + Temperature variation due to heat conduction among neighbouring rooms + Heating from internal sources like computers , lights, printers etc. (in watts) + Heating from people in the room (in watts) + Temperature change due to air conditioning contribution.


So, the equation for cooling in the rooms will look like this:


Total heat flow in the room, $\dot{Q}_i^{total}= C_i \frac{dT_i}{dt}$
$$= a_{ext}(T_{ext}(t)-T_i (t)) +a_{rooms} \sum_{j \in neighbours}^{} (T_j(t)-T_i(t))$$ 
\begin{equation} \label{eq:1}
 + \dot{Q}_{internal} + \dot{Q}_i^{mob}(t) + \rho \dot{V}_{HVAC} C_p (T_{HVAC}(t)-T_i(t)) u_i(t)
\end{equation}
where,

$C_i$ is the Heat Capacity of room $i$.

$\frac{dT_i}{dt}$ is the rate of temperature change in room $i$.

$T_i (t)$ is the Temperature of room $i$ at time $t$.

$a_{ext}$ and $a_{rooms}$ are constants related to heat conduction.

$T^{external} (t)$ is the ambient temperature at time $t$.

$\dot{Q}_{internal}$ is the heating due to internal devices. We have considered this constant across all rooms in a building.

$\dot{Q}_i^{mob}(t)$ is the heating due to mob present in the room $i$ at time $t$.

$\rho$ is the air conditioning air density.

$\dot{V}_{HVAC}$ is (volume/time) of cool air coming in. We have considered this constant across all rooms.

$C_p$ is the specific heat capacity of cool air.

$T_{HVAC}$ is the temperature of cool air. For bigger rooms, we have considered cool air having lower temperature.

$u_i(t)$ is the air-condition controller input( mainly ON/OFF).

Now we go into the details of each term and assumptions made for each term one by one.

\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=5cm]{tex.png}
    \caption{July,2019 daily ambient external temperature data in Marceed, CA. Average daily temperature in Marceed, CA in red dots. }
    \label{fig:tex}
\end{figure}
\textbf{(i) Generation of $T_{ext}(t)$}: Generation of External ambient temperature is a bit tricky because temperature varies a lot depending on the season, daily time and place. For this simulation, we have focused on cooling mainly. Therefore, we are simulating an environment where the ambient temperature is relatively higher so that the cooling system can trigger. We could have generated a Multivariate Normal Distribution with non-trivial co-variance matrix to generate the ambient temperature. But to include a practical real world experience, we have considered the ambient temperature data of Marceed, California during summer time. We have taken the average temperature at each moment(actually at time step, $\Delta t= 5$ minutes interval) for 10 hours daily over 1 month data. Fig. \ref{fig:tex} will demonstrate the whole July,2019 data from 9:00 to 19:00 and also show the average ambient temperature at each time step. The mean and standard deviation of the average data are 85F and 4.33 respectively. The data can be found from \cite{bell2013us}.

\textbf{(ii) Generation of $\dot{Q}_{internal}$}: This term is responsible for heat generation inside the rooms. Typically, we can see 3 computers, 1 printer, 4 light bulbs in a room. The temperature contribution by these devices is presented in Section \ref{subsec:supli1}. Other heating sources, such as Heaters, may also be present inside the rooms. But as we have stated earlier, since we are simulating a `Cooling down' environment, we are ignoring the Heater in this simulation. Nonetheless, our map Reconstruction Algorithm, discussed in Section \ref{sec:3}, can detect other possible heating sources if present.

\textbf{(iii) Generation of $\dot{Q}_i^{mob}(t)$}: This term refers to the heat generation from the occupants' body. We have considered that the number of people in a room is \textit{constant} for an hour. That means, after people come inside an office room, they do not go out at least for an hour. This time (here 1 hour) is called \textit{Time Range\textbf{(TR)}} between which mob number stays \textit{constant} at every room. More about TR is discussed in \ref{sec:4}. Also, for now, we are assuming that total number of people, $N$, in all $k$ rooms of the building is fixed over any time. That means, if the number of people in room $i$ at time $t$ is $n_i(t)$ then:
\[
    \sum_{i=1}^{k} n_i (t) = N\\
\]

Now, the heat contribution by the mobs in room $i$ , 
$$\dot{Q}_i^{mob}(t) = \sum_{m=1}^{m=n_i(t)} <q_m>$$
where, $<q>$ is the emitted energy distribution from mobs' body [$<q>=Gaussian(\mu = 110W, \sigma=1$)]

\textbf{(iv) Generation of $n_i(t)$}: Let, number of big conference room = BCR; number of small conference room = SCR and number of office rooms = OR. In our simulation model, we have assumed that BCR=1; SCR=1 and OR=14.

Let, the number of people staying in room $i$ will depend on some weight, $w_i$. [ to simulate the situation that conference rooms generally contain more people than the office rooms] 

So, the probability that a person will stay in room $i$ = $\frac{w_i}{\sum_{i} w_i}$ where, weight vector, $W = [w_1,w_2,......., w_N] = w_{1}^{b},w_{BCR+1}^{s}, w_{BCR+SCR+1}^{o}....,w_{N-BCR+SCR}^{o}.  $
Here, $w_{i}^{b}$ is the weight for big conference room, $w_{i}^{s}$ is the weight for small conference room and $w_{i}^{o}$ is the weight for office rooms. Choice of $W$ is mentioned in \ref{subsec:supli2}.\newline

\textbf{(v) Generation of $T_{HVAC}$}: We have assumed that the HVAC supplies cool air with temperature \textit{constant} over the times but variable across rooms. For instance, in our simulation, we have considered $T_{HVAC}$ = 50F for  big conference room and 55F for small conference or office rooms.

\textbf{(vi) Generation of $u_i(t)$}: This term refers to the ON/OFF state of HVAC's AC system. Depending on the current temperature of a room, the HVAC can trigger the AC system. Usually the occupants prefer their room temperature in a comfortable range. Therefore, the set points of room temperatures $T_i \in [T_i^{min}, T_i^{max}]$ and depending on that the AC controller input:
\[
    u_i(t)= 
\begin{cases}
    1,& \text{if } T_i\geq T_i^{max}\\
    0,& \text{if } T_i\leq T_i^{min}\\
    u_i(t-1),              & \text{otherwise}
\end{cases}
\]

where, $[T_i^{min} , T_i^{max}]$ is the temperature range in the rooms. 

\textbf{Final Simulation: }So far we have described the details about various factors present in Eq. (\ref{eq:1}). More details and calculations of these factors are given in \ref{subsec:supli1} and \ref{subsec:supli2}. Now, if we rewrite Eq. (\ref{eq:1}), the final equation that we are going to use looks like this:
$$\frac{T_i(t+1)-T_i(t)}{\Delta t} = \alpha (T_{ext}(t)-T_i (t)) + \beta \sum_{j \in X}^{} (T_j(t)-T_i(t)) +$$
\begin{equation} \label{eq:2}
 +  \omega + \gamma * M_{i}^{mob}(t) + \phi (T_{HVAC}(t)-T_i(t)) u_i(t)
\end{equation}
where,

$X$ is the set of neighbour rooms of room $i$.

$\alpha = \frac{a_{ext}}{C_i}$,$\beta = \frac{a_{rooms}}{C_i}$,$\omega = \frac{\dot{Q}_{internal}}{C_i} $,$\gamma = \frac{1}{C_i}$

$M_{i}^{mob}(t)=\sum_{m=1}^{m=n_i(t)} <q_m>$

$\phi = \frac{\rho \dot{V}_{HVAC} C_p}{C_i}$\newline

$\frac{dT_i}{dt}=\frac{T_i(t+1)-T_i(t)}{\Delta t}$ where $\Delta t$ is the time step which is the interval at which the sensor data is collected.

One thing to mention that we have performed 10 hours of
simulation. The time unit in our simulation will be in hour(h). Also we have run our simulator with all the temperature values in Kelvin($K$). For better understanding, we are mentioning the temperatures in Fahrenheit(F) in this paper. Finally, running our simulation, considering the parameters mentioned above and in \ref{subsec:supli1} and \ref{subsec:supli1}, the resulting outcomes following Eq. (\ref{eq:2}) can be viewed from Fig. \ref{fig:room1sensortempheattransfer}. The building architecture for our work is presented in Fig \ref{fig:architecture} as well.
\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=5cm]{architecture1.png}
    \caption{Architecture of the building for our simulation where we have a total of 16 rooms (Room 1- Big Conference room, Room 16- Small Conference room, Room 2 to 15- Normal Office room). We have assumed that Room 6,7,10 and 11 can exchange heat with only neighbouring rooms where as other rooms can exchange heat between both ambient and neighbouring rooms.}
    \label{fig:architecture}
\end{figure}

\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=5cm]{simulation1.png}
    \caption{Big conference room (Room 1) and  Office Room's (Room 2) Sensor Temperature Reading from our simulation (above) and other simulation factors such as mob distribution (mid) and AC controller input(below - 1 means ON).}
    \label{fig:room1sensortempheattransfer}
\end{figure}

From Fig. \ref{fig:room1sensortempheattransfer}, we can see that the temperatures are remaining between the set points (70F and 80F). Similar kind of behavior was observed in Ref. \cite{privara2013building} and \cite{hazyuk2012optimal} with a slight variation as we have taken building occupants and some other extra factors into account. Therefore, we can be confident that the temperature data from our simulation is completely valid.

\textbf{Problem formulation: }Now that we have simulation data of room temperatures in our hand, our problem formulation will be very easy. If we are given the temperature data of rooms and environment from temperature sensors, containing Gaussian noise, and AC's states from AHU sensors, using some known constants, \textbf{``Can we infer $M_{i}^{mob}(t)$ which is equivalent to infer $n_{i}^{mob}(t)$ correctly''?}  









%%%%%%%%%%%%%%%%% METHOD DESCRIPTION %%%%%%%%%%%%%%%%%%%%%


\section{\label{sec:3}Our Method to Infer Mob Map}
At this point we have our problem formulation. In this section, we will describe our map \textbf{Reconstruction Algorithm (RA)}. As stated earlier, our Algorithm is based on a variation of Least Square Estimator(LSE) with $L_2$ Regularization. LSE gives us our desired $M_{i}^{mob}(t)$ from which we can infer $n_{i}^{mob}(t)$ and $L_2$ regularization ensures the fact that the mobs stay at the same room for quite a moment. Now we will explain the development of our Algorithm step by step from the next paragraph.

\textbf{Development of our method: }If we rewrite Eq. (\ref{eq:2}) in matrix format for $k$ rooms and dividing it to L.H.S. and R.H.S we get:

L = $\frac{\Bar{T}(t+1)-\Bar{T}(t)}{\Delta t}$

R = $\alpha I  (\Bar{T}^{external} (t)-\Bar{T} (t)) + \beta I \sum ( \Bar{T}^{neighbour} (t) -\Bar{T} (t)) + \omega +  \gamma I \Bar{M}^{mob} (t) - \phi I (\Bar{T}_{HVAC}(t)- \Bar{T}(t)) \Bar{u}(t)$

The known things in our method are $C_i , \gamma, \phi$ and all other things are unknown. Among the unknowns, we are assuming that we can measure $ u_i$ (HVAC ON/OFF) without any noise. But this is not the case for $T_{HVAC}, T_i , T_{j \in Neighbour}$ and $T_{ext}$. So, assuming that we have some independent sensors which can measure these values with some Gaussian noises like:
\[
    \Bar{T}_{sensor} = \Bar{T} + Noise(\Bar{\eta})%\text{ and }
    %\Bar{T}_{sensor}^{external} = \Bar{T}_{ext} + \Bar{\eta}\\
\]
and put them in Eq. (\ref{eq:2}), we will get $L = R+ \eta$.
Therefore, if we want to find the Mob Map, we need to estimate the model parameters. For this, we will be using Least Square Estimation to decouple the noise ($\eta$) and optimize the model parameters $\alpha, \beta, \omega$ and $ \gamma \Bar{M}^{mob} (t)$. The procedure will look like this:
\begin{equation}\label{eq:3}
\begin{aligned}
& \underset{\alpha, \beta, \omega, \gamma \Bar{M}^{mob} (t) }{\text{argmin}}
& & \left\lVert L-R \right\rVert_{2}^{2} \\
& \text{s.t.} & &  \sum_{i=1}^{K} \gamma M_i^{mob}(t) = N*<\dot{q}>* \gamma \\
& & & \gamma* M_i^{mob}(t)\geq 0, \;  \forall i,t \\
\end{aligned}
\end{equation}

where $<\dot{q}>$ is the average energy emitted from a mob body. Now if we add $L_2$ Regularization term with (\ref{eq:3}) we can impose the situation where the number of mob remains almost same between two consecutive time steps.

\begin{equation}\label{eq:4}
\begin{aligned}
& \underset{P}{\text{argmin}}
& & \left\lVert L-R \right\rVert_{2}^{2}+\sum_{i=1}^{K}\sum_{t} \lambda \Bigg(M_i^{mob}(t+1)- M_i^{mob}(t)\Bigg)^2 \\
& & &   \\
\end{aligned}
\end{equation}
s.t. above constraints in (\ref{eq:3}). Here, $P=$ {$\alpha$, $\beta$, $ \omega$, $\gamma \Bar{M}^{mob} (t)$} and $\lambda = 0.1$.

The choice of $\lambda$ will be discussed in Section \ref{sec:4}. One thing to mention that if we have $k$ rooms and $z$ number of time steps (meaning that for each room we have collected the sensor data for z times at $\Delta t$ time interval, there are $P=k*z$ equations in this system. But we have $Q=k*z+3$ parameters to optimize. That means as P gets bigger, we get $P \approx Q$ which suggests that LSE will yield better convex solutions. 

\textbf{Relaxing the constraint: } We now focus on relaxing the constraint. The constraint in Eq. (\ref{eq:3}) mainly imposes that we need to know the exact total number of people inside the building to get the Mob Map which is hard to know. At most we can have a good guess on the total number of people in the building. We, now, rewrite this constraint in Eq. (\ref{eq:3})  which gives us the Mob Map if we can have a close guess on the total number of mob.
\begin{equation}\label{eq:5}
\begin{split}
N_{min}*\gamma<\dot{q}> \leq\sum_{i=1}^{K} \gamma M_i^{mob}(t)\leq N_{max}*\gamma <\dot{q}> =>\\
(1-\epsilon_2)N*\gamma<\dot{q}> \leq\sum_{i=1}^{K} \gamma M_i^{mob}(t)\leq (1+\epsilon_1)N*\gamma <\dot{q}>
\end{split}
\end{equation}
where, $\epsilon_1,\epsilon_2\geq0$. So, even if we specify a range of total mob, $[N_{min},N_{max}]$, in this constraint, we still get a reliable Mob Map. Note that if $\epsilon_2>1$, we have ignored the $(1-\epsilon_2)N*\gamma<\dot{q}>$ part because energy can not be negative. The effect of choosing $\epsilon_1$ and $\epsilon_2$ will be demonstrated in Section \ref{sec:4}.

However, we have now all the ingredients in our hand to run the estimator and it gives us the optimized parameter $\gamma \Bar{M}^{mob} (t)$ . The final rule used by our Reconstruction Algorithm to get $n_{i}^{mob}(t)$ is given below:
\begin{equation}\label{eq:6}
\text{Mob Map, }n_{i}^{mob}(t)=\text{Round to Integer}\left(\frac{\gamma* \Bar{M}^{mob} (t)}{\gamma * <\dot{q}>}\right)
\end{equation}

It can easily be seen that the performance of our Reconstruction Algorithm depends on $\epsilon, \lambda \text{ and } \eta$ whose effect will be discussed in Section \ref{sec:4}.









%%%%%%%%%%%%%%%%%%%%% RESULTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\label{sec:4}Results}
Now that we have described our Simulation, Problem Formulation and our Reconstruction Algorithm (\textbf{RA}), in this section, we show-case the output and performance of RA as well as the effect of various model parameters ($\epsilon, \lambda \text{ and } \eta$). 

\textbf{Output of RA applied on simulated temperature data: }
If we apply RA on the simulated data using Eq. (\ref{eq:4}) and (\ref{eq:6}), we can successfully recover the  model parameters, $\alpha, \beta, \omega, \gamma M_i^{mob}(t)$ and finally get $n_i^{mob}(t)$. We have recovered:

$$\alpha = 0.099  \text{ , } \beta = 0.101 \text{ and } \omega = 1.35$$ which is almost exact to the parameters used in simulation.

\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=6cm]{noisevsinference.png}
    \caption{Big conference room's (Room 1) Mob Map from simulated model and inferred parameter from RA at each hour for (a) Noise std, $\eta_{std}=10$  (b) $\eta_{std}=1$ (c) $\eta_{std}=0.1$ (d) $\eta_{std}=0.01$ [K=16, N= 45, BCR=1, SCR=1, OR=14 , $\Delta t=1 minute$, $z=600$, $TR=1$ hour, $\lambda=0.1$, $\epsilon=0.2$]}
    \label{fig:mobmapsunburstheattransfer}
\end{figure}


Fig. \ref{fig:mobmapsunburstheattransfer} demonstrates our constructed Mob Map, $n_i^{mob}(t)$, using Eq. (\ref{eq:6}) with the variation of noise. Note that, originally, for a room, we get the number of people at each time step. But usually people do not move from one room to another very often. For this, we defined \textit{Time Range(\textbf{TR})}, consisted of multiple time steps, in between no mob moves from one room to another. In our simulation, we assumed that mobs stay in one room for one hour, setting TR=1hour. So, in the final Mob Map construction, we took the Median of mob number over one hour. That is how we got one single mob number for each hour in Fig. \ref{fig:mobmapsunburstheattransfer}. When we implemented RA on real data set, we set TR=30 minutes and yet got reasonable mob map (shown later of this Section). In RA, TR can be set to any value depending on the situations and applications. However, we can see from Fig. \ref{fig:mobmapsunburstheattransfer} that when the standard deviation of noise is very high ($\eta_{std}=10$) in (a), the optimizer works very bad to infer the mob number. But as long as we decrease $\eta_{std}$ in (b), (c) and (d), the inference tends to match with the number of mob from our simulation. And finally at (d), when the $\eta_{std}=0.01$, the inferred mob number and simulated mob number are close to be matched.    

\textbf{Performace evaluation of RA: }
We measure the inference performance of RA by a term called \textit{Total Reconstruction Error \textbf{(TRE)}} which is a function of \textit{Normalized Mean Absolute Error \textbf{(NMAE)}}. The lower the TRE is, the better the performance is. We define TRE and NMAE as follows:

\[
    \text{TRE} = \frac{\sum_{i}^{k} \text{NMAE}_i}{k}\\
\]
\[
    \text{NMAE}_i = \frac{\text{Mean}(|Mob_{simulated} - Mob_{inferred}|_{\forall t})}{\text{Mean }Mob_{simulated} \text{ in room }i}\\
\]
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=4cm]{noisevserror.png}
    \caption{TRE of RA vs $Log_{10}$ of $\eta_{std}$ [K=16, N= 45, $\Delta t=1$ minute, $z=600$, $\lambda=0.1$, $\epsilon=0.2$].  }
    \label{fig:mobmapNMAEheattransfer}
\end{figure}
We measure the performance of RA on the basis of TRE with respect to the variation of the model parameters (i)$\eta_{std}$ ,(ii)$\lambda$ and (iii) $\epsilon$.

\textbf{(i) Effect of $\eta_{std}$ on TRE: }
Fig. \ref{fig:mobmapNMAEheattransfer} exhibits the effect of  $\eta_{std}$ (actually $Log_{10}$ of $\eta_{std}$)  on the performance of RA in terms of TRE. When $\eta_{std}\leq 1$ ($\leq $0 along X axis), we get TRE $\leq 0.2$ which is similar to having maximum 20\% error in reconstruction. If we consider that as our tolerance level, we can allow maximum Gaussian noise with standard deviation 1. Beyond that standard deviation, the reconstruction performance will degrade largely. Therefore, we recommend the level of accepted $\eta_{std}$ in range [0,1] to have a reliable Mob Map. 

\textbf{(ii) Effect of $\epsilon$ on TRE: }In Section \ref{sec:3}, we mentioned that our inference performance varies depending on the choice of $\epsilon_1$ and $\epsilon_2$ in constraint (\ref{eq:5}). We will show the effect of choosing $\epsilon_1$ and $\epsilon_2$ by considering $\epsilon_1=\epsilon_2=\epsilon$ which is equivalent to setting constraint $(1-\epsilon)N*\gamma<\dot{q}> \leq\sum_{i=1}^{K} \gamma M_i^{mob}(t)\leq (1+\epsilon)N*\gamma <\dot{q}>$. In Fig. \ref{fig:epsilonvstre}, we have shown the effect of $\epsilon$ on TRE. It is evident from Fig. \ref{fig:epsilonvstre} that choosing small range of $[N_{min},N_{max}](\epsilon \approx 0)$, closer to the actual total mob in the building yield better map reconstruction (lower TRE).  $\epsilon=0$ is equivalent to using the constraint in (\ref{eq:3}) as if we know the exact number of people in the building and in this case, the TRE is the lowest. Having $\epsilon>2$ is actually equivalent to using no constraint at all. So, the lower the $\epsilon$ be, the better the performance of RA be.  
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=4cm]{epsilonvstre.png}
    \caption{TRE of RA vs $\epsilon$ [K=16, N= 45, $\Delta t=1 minute$, $z=600$, $\lambda=0.1$, $\eta_{std}=0.1$].}
    \label{fig:epsilonvstre}
\end{figure}

\textbf{(iii) Effect of $\lambda$ on TRE: }The last thing we want to discuss is the effect of $\lambda$ on map reconstruction performance. From the empirical result shown in Fig. \ref{fig:lambdavstre}, we see that when $\lambda=0.1$, we get the lowest TRE, meaning better reconstruction. We recommend to use  $\lambda=0.1$ but depending on the recommended max tolerance level (20\%), $\lambda$ can have a value in range $\lambda=[0.03,0.3]$
\begin{figure}[htp]
    \centering
    \includegraphics[width=9cm, height=4cm]{lambdavserror.png}
    \caption{TRE of RA vs $\lambda$ [K=16, N= 45, $\Delta t=1$ minute, $z=600$, $\epsilon=0.2$, $\eta_{std}=0.1$].}
    \label{fig:lambdavstre}
\end{figure}

\textbf{Implementation on Real Data set:}
As we have mentioned earlier, no data set is complete to run our method. That is why we choose to simulate the room temperatures. Till now we have seen the performance of RA on the simulated data. However, to show the effectiveness of RA in different scenario, we are implementing our method of RA to some real toy data sets. We assume reasonable values for the missing arguments for our Algorithm.

\textbf{(i) Data set 1:} This data, in \cite{armknecht2019privacy}, was collected from March to April, 2016. We have filtered the data set to get 10 hours of data(sampled every 3 minutes) from April 28, 2016 . It contains the temperature of only one room as well as the number of occupants in that room. As a consequence, we get ground truth to compare our results. The only problem of this data set is that we do not have some other distributions like ambient temperatures and HVAC status (ON/OFF or cool air temperature). We assume reasonable values for these. For example, we set $T_{ext}(t)$ from a distribution $(\mu=55F, \sigma=2)$ which is compatible with ambient temperature in Mannheim, Germany from where the data was collected. Another thing is that because of the average ambient temperature being very cool($\mu=55F$), we assume that the air conditioner is OFF. Considering these situations in mind, we have applied RA on this data set and got the Mob Map like in Fig. \ref{fig:germany}. Moreover, the relative higher value of $\omega = 2.31$ (in our simulation $\omega \text{was} 1.36$) delivered by RA indicates the presence of possible Heating System inside the room. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=4cm]{mobmap_germany.png} 
    \caption{Mob Map generated from Data set 1 ($TR=30$ minutes). At each TR, left column is our inferred mob number and right column is the actual mob number.[$\Delta t=3$ minutes, $z=200$, $\epsilon=0.2$, $\lambda=0.1$]}
    \label{fig:germany}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=8cm, height=4cm]{mobmap_house.png} 
    \caption{Mob Map generated from Data set 2 ($TR=30$ minutes).[$\Delta t=3$ minutes, $z=200$, $\epsilon=0.2$, $\lambda=0.1$]}
    \label{fig:house}
\end{figure}

\textbf{(ii) Data set 2:} We have filtered this data set in \cite{candanedo2017data} to collect 10 hours (9:00 to 19:00) of data sampled in every 10 minutes from May 26, 2016. The room architecture (neighbour room information) is known and we have gathered the data of all four rooms in lower floor. However, we can get $T_{ext}(t)$ and $T_i(t)$ directly from the data set. To get an idea of AC's ON/OFF status, we have observed that, for Room 3, the temperature dropped abruptly from 11:00 to 12:30 and from 14:00 to 17:00. We have assumed that in this time the AC was ON. Another thing is that there was no hints given about HVAC's air volume capacity or temperature of the cooled air. For this, we have used the values of $\phi$ and $T_{HVAC}$ from our simulation. Considering these assumptions, we have run RA on this data set and got the Mob Map of Room 3 similar to Fig. \ref{fig:house}. Note that there is no ground truth on the number of occupant in this data set. We have chosen Room 3 to show the Mob Map here because this room is attached with Room 1 and Room 2 as well as with the environment which is almost similar to our simulation design.  


%%%%%%%%%%%%%%%%%%%%%%%% DISCUSSION AND CONCLUSION %%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\label{sec:5}Discussion and Conclusion}
In this paper, we have simulated a thermal modeling of a building and proposed a method to infer the Mob Map. We have found out that if we have access to a particular room temperature, temperature of its neighbourhood rooms as well as AC's control dynamics such as ON/OFF status and cooled air temperature, we can easily infer a reliable Mob Map. Not only that, we also demonstrate the applicability and performance of RA in terms of Total Reconstruction Error with respect to the variation of various factors such as noise level from sensor data, choice of the constraint and other model parameters ($\epsilon , \lambda$) etc. Moreover, we have illustrated the effectiveness of our Algorithm by applying it on two test data sets. Still there are possible spaces for further development. In future, we will apply our method on a real data set compatible with our method. Another thing to mention that though our simulation model is moderately complex, there is still room for constructing more complex and realistic thermal model, for instance , accumulating solar radiation and heat transfer via convection.  





%%%%%%%%%%%%%%%%% SUPLIMENTARY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{\label{sec:6}Supplementary Materials}
\subsection{Choice of the Constants:}\label{subsec:supli1}
\textbf{$C_i$}: $C_i$ is the Heat Capacity for entire room. All the elements (air, furniture and walls) in a room contribute to it.
$$C_i= C_{air} + C_{furniture} + C_{wall} = (C_{volumetric}* volume) +$$ 
$$+(\text{Furniture mass * Specific Heat Capacity,}C_p ) + $$
$$+(\rho_{wall}*volume_{wall}*(C_p)_{wall})$$
Considering standard values, we get,
$$C_i=(1.29KJm^{-3}K^{-1} * 30m^3) + (4200 J/kgK * 200kg) +$$ $$+(2.13*10^5 gm^{-3}*5m^3*0.84 J/gK) = 1*10^6 J/K$$
$a_{ext}$: Every room performs heat transfer with the ambient temperature via conduction process in the wall and window glass. The equation for $a_{ext}$ is:
$$a_{ext} = h_{wall}*A_{wall} + h_{glass}*A_{glass}$$
where, h is the Thermal Transmittance of a substance. Using standard values we get:
$$a_{ext} = (1Wm^{-2}K^{-1} * 20m^2)+(5Wm^{-2}K^{-1} * 2m^2) = 30W/K$$

$a_{room}$: Every room performs heat transfer with neighbouring rooms via conduction process in the wall only. The equation is same as $a_{ext}$ but excluding the glass part. Using standard values we get:
$$a_{rooms} = (1Wm^{-2}K^{-1} * 20m^2) = 20W/K$$\newline


$\dot{Q}_{internal}$: Considering 3 computers (100W energy consumed per computer), 4 lights (10 W per light) and 1 printer(40W/printer) per room, each room will radiate a total of 380W = $1.36*10^6$J/h energy.\newline

$<\dot{q}>$: Average heat produced by an average human body while staying indoor is given by the equation:
$$<\dot{q}> = M*A_{body}$$
Considering standard Metabolic rate, $M = 55Wm^{-2}$ and average body area, $A_{body} = 2 m^2$ we get, $<\dot{q}> = 110W = 3.96*10^5 J/h$\newline

$\rho \dot{V}_{HVAC} C_p$: Considering each room 250 sqr-ft and standard rules of 1 Cubic ft per minute (1 CFM) per sqr-ft, we get $\dot{V}_{HVAC} = 250 CFM = 450 m^3/h$. Using usual values, we get $\rho \dot{V}_{HVAC} C_p$ = $\rho_{air} \dot{V}_{HVAC} (C_p)_{air}= 1.225 kgm^{-3} * 450 m^3/h *  1000 J/kgK = 5.51*10^5 J/hK$


Now,
$\alpha = \frac{a_{ext}}{C_i} = \frac{30W/K}{10^6 J/K}= 0.1h^{-1}$

$\beta = \frac{a_{rooms}}{C_i} = \frac{20W/K}{10^6 J/K}= 0.1h^{-1}$

$\omega = \frac{\dot{Q}_{internal}}{C_i} = \frac{1.36*10^6J/h}{10^6 J/K}=1.36 Kh^{-1}$

$\gamma = \frac{1}{C_i} = \frac{1}{10^6 J/K}= 10^{-6} K/J$

$\phi = \frac{\rho \dot{V}_{HVAC} C_p}{C_i} = \frac{5.51*10^5 J/hK}{10^6 J/K}= 0.6h^{-1}$\newline

\subsection{Simulation Parameters:}\label{subsec:supli2}

$\alpha = 0.1h^{-1}$, $\beta = 0.1h^{-1}$, $\omega =1.36 Kh^{-1}$, $\gamma = 10^{-6}KJ^{-1}$, $\phi = 0.6h^{-1}$

$[T_i^{min},T_i^{max}] = [70F, 80F]$

Total number of rooms, $k$ = 16 and Total mob in the building, $N$ = 45 [Distributed over $k$ rooms]

Number of Big Conference room, BCR = 1; number of Small Conference room, SCR = 1; number of Normal Office room, OR = 14.

Weight for Big conference room, $w_{i}^{b}$ = 5; weight for small conference room, $w_{i}^{s}$ = 3; weight for office room, $w_{i}^{o}$ = 1

Total time for simulation = 10 hours; time step for solving the equation, $\Delta t$ = 10/600 hour = 1 minute; Time range, $TR=1$ hour.

\subsection{Implementation Platform Details:}\label{subsec:supli3}
We have used Python platform (Python 3.7.2) and SQSLP optimization algorithm from  scipy package in order to manipulate the LSE and $L_2$ Regularization to  optimize the model parameters. All the codes were run in Macbook Pro, 2017, 2.3 GHz Intel Core i5, 16 GB memory. 

